A new analysis technique to measure the W Production Charge Asymmetry at the Tevatron

We propose an analysis technique to directly measure W production charge asymmetry from W leptonic decay events at the Tevatron and show the feasibility for new analysis method using Monte Carlo simulations.

==> Makefile <==
###############################################################################
#                                                        December 4, 2002
#
# Makefile for a sample CDF Note - Stefan Stonjek  <s.stonjek@physics.ox.ac.uk>
#                                  Martin Hennecke <hennecke@fnal.gov> 
#
###############################################################################

tex_main      = WAsym_prdrc
tex_files    := $(wildcard *.tex)

graphics_eps := $(wildcard *.eps)
graphics_pdf := $(patsubst %.eps,%.pdf,$(wildcard *.eps))

ps: $(tex_main).ps
	gv -scale 1 $(tex_main).ps  

pdf: $(tex_main).pdf
	acroread $(tex_main).pdf & 

$(tex_main).pdf: $(tex_files) $(graphics_pdf)
	pdflatex $(tex_main).tex && pdflatex $(tex_main).tex && thumbpdf $(tex_main) && pdflatex $(tex_main).tex

$(tex_main).ps: $(tex_files)
	latex $(tex_main).tex && latex $(tex_main).tex && dvips $(tex_main).dvi -o 

%.pdf: %.eps
	epstopdf $< -o $@

.PHONY: clean
clean:
	rm -r -f *.aux *.dvi *.log *.out *.pdf \
	*.ps *.toc *.tof *.tpt *.end thumb*.* *~ $(graphics_pdf)

